FedBlock: A Blockchain Approach to Federated Learning against Backdoor Attacks

Federated Learning (FL) is a machine learning method for training with private data locally stored in distributed machines without gathering them into one place for central learning. Despite its promises, FL is prone to critical security risks. First, because FL depends on a central server to aggregate local training models, this is a single point of failure. The server might function maliciously. Second, due to its distributed nature, FL might encounter backdoor attacks by participating clients. They can poison the local model before submitting to the server. Either type of attack, on the server or the client side, would severely degrade learning accuracy. We propose FedBlock, a novel blockchain-based FL framework that addresses both of these security risks. FedBlock is uniquely desirable in that it involves only smart contract programming, thus deployable atop any blockchain network. Our framework is substantiated with a comprehensive evaluation study using real-world datasets. Its robustness against backdoor attacks is competitive with the literature of FL backdoor defense. The latter, however, does not address the server risk as we do.

==> 05_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

This section provides discussion on miscellaneous related issues to the proposal and it highlights some of its limitations.








==> additional.tex <==
\section{Additional Work}\label{sec:additional}
\begin{document}

\vspace{1cm}


\end{document}

==> macro.tex <==
\newcommand{\tbhline}{\noalign{\hrule height 1pt}}
\newcommand\inner[2]{\langle #1, #2 \rangle}

\newcolumntype{|}{!{\vrule width 0.5pt}}
\newcolumntype{?}{!{\vrule width 1pt}}
\newcolumntype{^}{!{\vrule width 1.2pt}}


\renewcommand{\O}[1]{$\mathcal{O}(#1)$}


\newcommand{\bhline}[1]{\noalign{\hrule height #1}}    
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}    

%\renewcommand{\theenumi}{\ajMaru{enumi}}


% remove end sentences
\algtext*{EndWhile}
\algtext*{EndIf}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\Break}{\textbf{break}}

\newcommand{\argmax}{\mathop{\rm arg~max}\limits}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\newcommand{\twoKperf}{20}
\newcommand{\fourKperf}{30}
\newcommand{\eightKperf}{2}

\newcommand{\iFDK}{\ding{iFDK}}%


% Nice little colorful numbered boxes
\definecolor{myblue}{RGB}{91,155,213}
\definecolor{mydark}{RGB}{0,0,0}
\newcommand*\circled[1]{\color{white}\tikz[baseline=(char.base)]{
		\node[shape=circle,inner sep=0.5pt,fill=myblue] (char) {#1};}\color{black}\,}
\newcommand*\circledempty[1]{\color{black}\tikz[baseline=(char.base)]{
		\node[shape=circle, draw=myblue, thin, inner sep=0.5pt,fill=white] (char) {#1};}\color{black}\,}
		
		
		
\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{cyan}\hl{#1}}}
\DeclareRobustCommand{\hllightgray}[1]{{\sethlcolor{lightgray}\hl{#1}}}
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}}


\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output\,}
\SetKwInOut{Data}{Data}
\SetKwProg{Tree}{Tree}{}{EndTree}


\newcommand{\rOne}{\ding{\rotatebox{90}{$256^2\times512\rightarrow256^3$}}}%
\newcommand{\rTwo}{\ding{\rotatebox{90}{$256^2\times512\rightarrow512^3$}}}%
\newcommand{\rThree}{\ding{\rotatebox{90}{$256^2\times512\rightarrow1024^3$}}}%
\newcommand{\rFour}{\ding{\rotatebox{90}{$512^2\times512\rightarrow256^3$}}}%
\newcommand{\rFive}{\ding{\rotatebox{90}{$512^2\times512\rightarrow512^3$}}}%
\newcommand{\rSix}{\ding{\rotatebox{90}{$512^2\times512\rightarrow1024^3$}}}%
\newcommand{\rSeven}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow256^3$}}}%
\newcommand{\rEight}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow512^3$}}}%
\newcommand{\rNine}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow1024^3$}}}%


\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\asteq}{\mathrel{*}=}


\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}



\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}

==> tables/change_L.tex <==
%\begin{table*}
%    \begin{minipage}[b]{0.5\linewidth}
\begin{table}[t]
        \centering
        \caption{Performance of FedBlock with $1000$ rounds as a result of varying the size $L$ of client verification set. Here, the number of clients in the smart contract that need verifying is fixed at $M = 30$ and the number of verifiers is fixed at $V=15$. The best results are highlighted in the \textbf{bold text}.}
        \label{table:optimalL}
        %\setlength\tabcolsep{3pt} % default value: 6pt
        \resizebox{\linewidth}{!}{%
            \begin{tabular}{c|c|c|c|c|c|c|c|c}
                \toprule
                \multirow{2}{*}{$L$
                %\centering \makecell[l]{Number of \\Clients/Verifier}
                } 
                & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c}{EMNIST} \\
                \cmidrule(lr){2-5} \cmidrule(lr){6-9}
                & {MA} & {BA} & {TPR} & {TNR} & {MA} & {BA} & {TPR} & {TNR} \\
                \midrule
                3 & 84.33 & 1.02 & 1.0 & 0.60 & 98.87 & 86.0 & 0.99 & 0.59 \\
                5 & 84.90 & 1.79 & 1.0 & 0.74 & 98.92 & 2.5 & 1.0 & 0.80 \\
                \textbf{7} &  \textbf{84.72} &  \textbf{1.87} & \textbf{1.0} &  \textbf{0.76} &  \textbf{98.91} & \textbf{3.0} &  \textbf{1.0} &  \textbf{0.84} \\
                9 & 84.98 & 2.30 & 1.0 & 0.77 & 98.93 & 5.0 & 1.0 & 0.85 \\
                11 & 84.74 & 1.78 & 1.0 & 0.76 & 98.92 & 5.5 & 1.0 & 0.84 \\
                \bottomrule
            \end{tabular}
        }
\end{table}
%\end{minipage}
    %\end{minipage}\hfill
    %\begin{minipage}[b]{0.3\linewidth}
    %    \centering
    %    \captionsetup{labelformat=empty}
    %    \includegraphics[height=3.5cm]{figures/optimalL.png}
    %    \captionof{figure}{Figure 2: Average True Negative Rate (TNR) for different values of $|\mathcal{L}|$ within 1000 rounds on CIFAR-10 and EMNIST.}
    %    \label{figure:optimalL}
    %\end{minipage}
%\end{table*}

==> tables/change_V.tex <==
%\begin{table*}
%    \begin{minipage}[b]{0.5\linewidth}
\begin{table}[t]
        \centering
        \caption{Performance of FedBlock with $1000$ rounds as a result of varying the number $V$ of verifiers. Here, the number of clients in the smart contract that need verifying is fixed at $M = 30$ and the size of client verification set is fixed at $L=7$. The best results are highlighted in the \textbf{bold text}.}
        \label{table:optimalV}
        %\setlength\tabcolsep{3pt} % default value: 6pt
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{c|c|c|c|c|c|c|c|c}
            \toprule
            \multirow{2}{*}{$V$
            %\centering \makecell[l]{Number of \\Clients/Verifier}
            } 
            & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c}{EMNIST} \\
            \cmidrule(lr){2-5} \cmidrule(lr){6-9}
            & {MA} & {BA} & {TPR} & {TNR} & {MA} & {BA} & {TPR} & {TNR} \\
            \midrule
            11 & 84.55 & 2.89 & 1.0 & 0.73 & 98.92 & 28.0 & 0.99 & 0.81 \\
            13 & 84.48 & 2.55 & 1.0 & 0.73 & 98.92 & 1.5 & 1.0 & 0.83 \\
            \textbf{15} & \textbf{84.72} & \textbf{1.87} & \textbf{1.0} & \textbf{0.75} & \textbf{98.91} & \textbf{3.0} & \textbf{1.0} & \textbf{0.84} \\
            17 & 84.72 & 2.55 & 1.0 & 0.75 & 98.96 & 4.0 & 1.0 & 0.85 \\
            19 & 84.77 & 2.21 & 1.0 & 0.75 & 98.93 & 4.0 & 1.0 & 0.85 \\
            \bottomrule
        \end{tabular}
        }
\end{table}       
%        \label{table:optimalL}
%    \end{minipage}\hfill
%    \begin{minipage}[b]{0.3\linewidth}
%        \centering
%        \captionsetup{labelformat=empty}
%        \includegraphics[height=3.5cm]{figures/optimalV.png}
%        \captionof{figure}{Figure 3: Average True Negative Rate (TNR) for different values of $|\mathcal{V}|$ within 1000 rounds on CIFAR-10 and EMNIST.}
%        \label{figure:optimalL}
%        \vspace{20pt}
%    \end{minipage}
%\end{table*}

==> tables/malicious_verifier.tex <==
%\begin{table}[h]
    \centering
    \small
    \captionof{table}{FedBlock %performance of FedBlock 
    against malicious verifiers (CIFAR-10,  $500$ rounds).
    }
    \label{table:ma_ver}
    %\vspace{0.2cm}
    %\setlength\tabcolsep{3pt} % default value: 6pt
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{l|l|l|l}
        \toprule
        & \textbf{\begin{tabular}[c]{@{}c@{}}Normal\end{tabular}} 
        & \textbf{\begin{tabular}[c]{@{}c@{}}Random \\Change\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Reverse \\Change\end{tabular}}  \\
        \midrule
        MA & 84.2 & 83.59 & 84.71 \\
        BA & 1.0 & 0.51 & 0.51 \\
        \midrule
        TPR & 1.0 & 1.00 & 1.00 \\
        TNR & 0.74 & 0.74 & 0.75 \\
        \bottomrule
    \end{tabular}
}
%\end{table}
